Lessons from the Use of Natural Language Inference (NLI) in Requirements Engineering Tasks

We investigate the use of Natural Language Inference (NLI) in automating requirements engineering tasks. In particular, we focus on three tasks: requirements classification, identification of requirements specification defects, and detection of conflicts in stakeholders' requirements. While previous research has demonstrated significant benefit in using NLI as a universal method for a broad spectrum of natural language processing tasks, these advantages have not been investigated within the context of software requirements engineering. Therefore, we design experiments to evaluate the use of NLI in requirements analysis. We compare the performance of NLI with a spectrum of approaches, including prompt-based models, conventional transfer learning, Large Language Models (LLMs)-powered chatbot models, and probabilistic models. Through experiments conducted under various learning settings including conventional learning and zero-shot, we demonstrate conclusively that our NLI method surpasses classical NLP methods as well as other LLMs-based and chatbot models in the analysis of requirements specifications. Additionally, we share lessons learned characterizing the learning settings that make NLI a suitable approach for automating requirements engineering tasks.

==> bert-background.tex <==
\section{Background}

% Transfer learning - BERT - NLI - Zero Shot - LLMs - ChatGPT
\subsection{Probabilistic text classification}
Probabilistic classifiers are machine learning techniques that use probability theory to assign class labels to input data points. These classifiers estimate the likelihood of a data point belonging to each possible class and then make a decision based on the highest probability. Previously, studies have employed probabilistic methods such as Naive Bayes~\cite{Abad:2017} for functional requirement (FR) and non-functional requirement (NFR) classification as well as an indicator terms-based approach~\cite{Cleland-Huang:EarlyAspects, Mirakhorli:Detecting} for classifying NFRs. 

% \subsection{Statistical Learning}
% Statistical learning approaches have enabled automated and accurate identification of requirements from unstructured textual data. Previously, several models have been developed for classifying NFRs~\cite{Cleland-Huang:EarlyAspects, Mirakhorli:Detecting}. In this work, we evaluate the performance of such models in classifying requirements.

% Transformation models are neural architectures that utilize self-attention mechanism to capture contextual dependencies within input sequence. These models operate by transforming the input through attention layers. 
% By incorporating the positional encoding and using attention mechanism they can capture the long-range dependencies.
% , which can be used in various software engineering tasks such as code generation, bug detection, and requirement classification, which can improve the software quality and reliability. 

\subsection{Transfer Learning}
% Transfer learning is a technique that utilizes knowledge acquired from one task to improve learning in another related task. 
% By leveraging understanding gained during the learning process of a source task, it enhances performance in a target task. 
% This approach is widely applicable in various domains, allowing models to adapt and excel in new tasks, even with limited data in the target domain.
% By the advent of transformation models, that utilize self-attention mechanism to capture contextual dependencies within input sequence, several language models have been developed.
% and utilized in the domain of software engineering, including requirement classification.
% Large Language Models (LLMs), also have been trained on massive dataset, and have shown promising results in various tasks. 
% Built on top of these LLMs, OpenAI's ChatGPT have been developed recently, that has been fine tuned with human annotated text, representing an interactive language model. While it has shown promissing results in various tasks, the aplicability of this model is yet to define in software requirement classification.

Transfer learning is a powerful technique that leverages knowledge gained from one task to enhance learning in another related task. By utilizing the insights acquired during the learning process of a source task, transfer learning significantly improves performance in a target task. 
Its broad applicability across various domains allows transfer learning models to adapt and excel in new tasks, even when faced with limited data in the target domain.
The advent of transformation models, which harness self-attention mechanisms to capture contextual dependencies within input sequences, has led to the development of several language models. 
Notably, large language models (LLMs) have emerged, trained on massive datasets, and exhibiting promising results across diverse tasks.
Among these advancements, OpenAI's ChatGPT has recently been developed, representing an interactive language model fine-tuned with human-annotated text. 
It has demonstrated promising performance in various tasks, yet its potential applicability in software requirements classification remains to be fully defined.

% \subsection{LLMs}

\subsection{Zero / Few Shot Learning}

One of the key limitations encountered in conventional machine learning approaches is their constraint to handle only the classes that have been previously observed during training.
Moreover, incorporating a new class into the model necessitates a substantial effort to retrain the entire model with additional samples. 
However, transfer learning, especially in the context of few-shot and zero-shot learning, offers the remarkable ability to adapt pre-trained models to previously unseen classes with limited or even no available data~\cite{brown2020language}.
This capability proves particularly advantageous in domains like software requirement engineering, where classes may evolve over time. 


\subsection{Prompt-based Mask Prediction}

Classification using masked prediction is a technique that formulates the classification problem as a masked language model problem~\cite{hu-etal-2022-knowledgeable}.
By formulating prompts that embed task-specific information alongside input data, the prompts act as guiding cues, steering the model towards learning the discriminative features crucial for successful classification. 
This allows the model to bridge the gap between the labels and the semantics of the labels.
By adding a prompt to every input and masking the class name, the model will be trained to predict the class that is masked within the given prompt. 
% Schick et. al. showed that by formulating the classification into a cloze question that contains the task description, the same performance could be achieved while working with much smaller language models~\cite{schick-schutze-2021-jus}.
% Meng et. al. showed that 
Schick et al.~\cite{schick-schutze-2021-just} demonstrated that formulating the classification as a cloze question containing the task description enables comparable performance even with significantly smaller language. 
This highlights the effectiveness and efficiency of prompt-based classification techniques.

\subsection{NLI}

NLI is a task aimed at determining whether a given sentence \textit{(hypothesis)} logically follows from another sentence \textit{(premise)}. Depending on their semantics, the possible outputs are categorized as \textit{entailment}, \textit{contradiction}, or \textit{neutral}. 
NLI has demonstrated remarkable performance in different scenarios, including conventional, few-shot, and zero-shot learning \cite{wang2021entailment}.
In our work, we reformulate the problem of classification into an inference problem. 
By integrating knowledge into the input samples through the means of providing a descriptive hypothesis, it empowers the NLI model to make more informed and contextually relevant inferences.
Besides this, we explored the potentials of integrating knowledge into the inference model by designing various hypotheses, and demonstrated the effect of the hypothesis on the requirements classification results.


%I added this section temporarily. We can move it to a different spot
% \st{
% Language models are 
% Bidirectional Encoder Representation from Transformers (BERT) \cite{devlin2019bert} is Language Model (LM). A LM estimates the probability of a sequence of words following a given sequence. LMs are commonly used to extract word embeddings where words and phrases are mapped to a vector of numbers that can be used for a variety of tasks.}

% \st{
% Early on, Recurrent Neural Networks (RNNs) such as Long Short Term Memory (LSTM) were used to solve Natural Language Processing (NLP) tasks. Word2vec \cite{Mikolovword2vec} and Global Vectors for Word Representation (GloVe) \cite{PenningtonGlove2014} were one of the most popularized LMs used for word embeddings. Both LMs were trained on a unlabeled corpus to learn relationships between words. However, both models are unidirectional and only learn one representation of words. 
% Embeddings from Language Models (ElMo) \cite{peters2018ELMo} is a bidirectional LSTM that uses generates embeddings based on the context of the words surrounding it. However, ELMo is only trained on words that it has seen before during training and needs to be trained from scratch for each domain. Universal Language Model Fine-Tuning (ULMFiT) \cite{howard-ruder-2018-ULFiT} introduces method for fine-tuning natural language models for transfer learning. }

% \st{
% The transfer learning model \cite{VaswaniAttention} is similar to LSTM in that they both use encoders and decoders, however, Transformer models rely on attention-mechanisms rather than RNNs. Transformers are categorized by having self-attention layers, position-wise feed-forward networks and positional encodings. OpenAI's Generative Pre-trained Transformer (GPT-2) uses self-attention from transformer model to learn better representations. However, OpenAI uses a unidirectional encoding method which means that it creates word embedding by looking at a sentence in one-direction. Bidirectional Encoder Representations form Transformers (BERT) is a language model that uses bi-directional word embedding.}

% \mehdi{Transformer-based model $->$ what does that mean for our experiment? Does it mean BERT is being fine tuned for our domain? How? also how transfer learning is used in our study? Maybe you can bring some text about transfer learning of BERT into  section IV where you talk about BERT again}

% BERT \cite{devlin2019bert} is a transformer-based pre-trained language model. BERT can be fine tuned for specific domains if it has enough data, or it can be used in its current state. BERT is trained bi-directionally on Wikipedia (https://wikipedia.com) and Book Corpora (https://yknzhu.wixsite.com/mbweb) datasets. During its training, BERT creates a large dictionary of words, sub-words, and characters, each with an assigned token ID.   
 
 % The BERT model breaks the data into tokens containing words, sub-words and characters with their associated IDs. A [CLS] token is inserted at the beginning of each requirement, and [SEP] tokens are inserted at the end of each sentence. The token IDs are stored in the hidden state. The hidden state references the tokens, the position of the tokens in relation to other words, the batch number (number of sentences), the feature number (dependant on the model used), and the layer number.
 

 
%  \begin{itemize}
%      \item Masked Language Modeling In this training technique, 15\% of input tokens are replaced by a [MASK] token and the model predicts the original token and creates embeddings corresponding to them. This helps train the model to learn relationships between different words.
% \item Next Sentence Prediction In this training technique, the model is given two sentences $A$ and $B$. The model needs to predict of sentence $B$ can logically follow sentence $A$. This helps the model learn relationships between different sentences. BERT has achieved high performance results on eleven NLP tasks \cite{ws-2018-2018}, and has performed well in non-functional requirement classification tasks \cite{Norbert_Hey}. We will be using BERT to classify security requirement sub-types. 
% \end{itemize}

 
%ELMO, ULMFit

%transformer architecture which uses encoder-decoder, stacked self-attention encoder-decoder structure. Multi-headed attention








